Integral Menger curvature for sets of arbitrary dimension and codimension

We propose a notion of integral Menger curvature for compact, $m$-dimensional sets in $n$-dimensional Euclidean space and prove that finiteness of this quantity implies that the set is $C^{1,\alpha}$ embedded manifold with the H{\"o}lder norm and the size of maps depending only on the curvature. We develop the ideas introduced by Strzelecki and von der Mosel [Adv. Math. 226(2011)] and use a similar strategy to prove our results.

==> ahlreg2.tex <==
\input{preambule.tex}
\input{macros.tex}

\title[Integral Menger curvature for sets of arbitrary dimension]
{Integral Menger curvature for sets of arbitrary dimension in $\Rn$.\\
  Part II: $C^{1,\alpha}$-regularity.}
\author{S{\l}awomir Kolasi{\'n}ski}
\address{Institute of Mathematics\\
  University of~Warsaw\\
  Banacha~2, 02-097 Warsaw\\
  Poland}
\email{s.kolasinski@mimuw.edu.pl}
\urladdr{http://www.mimuw.edu.pl/~skola}
\thanks{The author wishes to thank P. Strzelecki for his advice and many
  inspiring conversations.}
\keywords{Menger curvature, Ahlfors regularity, repulsive potentials}
\subjclass{Primary: 49Q10; Secondary: 28A75, 49Q20, 49Q15}
\date{\today}
\begin{document}

\begin{abstract}
  We propose the notion of integral Menger curvature for $m$-dimensional sets in
  $n$-dimensional Euclidean space and prove that finiteness of this quantity
  implies $C^{1,\alpha}$ regularity. We develop the ideas introduced by
  Strzelecki and von der Mosel [Adv. Math. 226(2011)] and use a similar strategy
  to prove our result.
\end{abstract}

\maketitle
% \tableofcontents

\section{Preliminaries}
\label{sec:prelim}

\input{prelim-grass.tex}
\input{prelim-cones.tex}
\input{prelim-flat.tex}
\input{prelim-adm-fine.tex}

\input{osctan.tex}
\input{imphol.tex}

\bibliography{menger}{}
\bibliographystyle{hplain}

\end{document}

% Local Variables:
% coding: iso-8859-2
% eval: (ispell-change-dictionary "american")
% eval: (flyspell-mode)
% End:

